Design and Scaffolded Training of an Efficient DNN Operator for Computer Vision on the Edge

Massively parallel systolic arrays and resource-efficient depthwise separable convolutions are two promising techniques to accelerate DNN inference on the edge. Interestingly, their combination is inefficient: Computational patterns of depthwise separable convolutions do not exhibit a rhythmic systolic flow and lack sufficient data reuse to saturate systolic arrays. We formally analyse this inefficiency and propose an efficient operator, an optimal hardware dataflow, and a superior training methodology towards alleviating this. The efficient operator, called FuSeConv, is a drop-in replacement for depthwise separable convolutions. FuSeConv factorizes convolution fully along their spatial and depth dimensions. The resultant computation efficiently maps to systolic arrays. The optimal dataflow, called Spatial-Tiled Output Stationary (ST-OS), maximizes the efficiency of FuSeConv on systolic arrays. It maps independent convolutions to rows of the array to maximize resource utilization with negligible VLSI overheads. Neural Operator Scaffolding (NOS) scaffolds the training of FuSeConv by distilling knowledge from the expensive depthwise separable convolutions. This bridges the accuracy gap between FuSeConv networks and baselines. Additionally, NOS can be combined with Neural Architecture Search (NAS) to trade-off latency and accuracy. The HW/SW co-design of FuSeConv with ST-OS achieves a significant speedup of 4.1-9.25X with state-of-the-art efficient networks for ImageNet. The parameter efficiency of FuSeConv and its significant out-performance over depthwise separable convolutions on systolic arrays illustrates their promise as a strong solution on the edge. Training FuSeConv networks with NOS achieves accuracy comparable to the baselines. Further, by combining NOS with NAS, we design networks that define state-of-the-art models improving on both accuracy and latency on systolic arrays.

==> content/background.tex <==
\noindent
\subsection{Systolic Arrays}

A systolic array \cite{kung1982systolic} is a parallel computing hardware, constituted of a large number of homogeneous Processing Elements (PEs). 
These PEs are interconnected in a regular arrangement, such as a rectangular grid, facilitating local communication with neighbours as shown in Figure \ref{fig:systolic}.  
The word `systolic' implies rhythmic patterns in communication and computation, which are globally synchronous.
This regular arrangement constraints how data flows amongst PEs thereby restricting the number of applications that can be mapped onto systolic arrays. 
However, embarrassingly parallel and regular applications such as matrix-multiplication can be directly mapped onto systolic arrays and have shown order of magnitudes higher performance over sequential hardware. 
The main benefits of systolic-arrays come from the nearest-neighbour communication leading to low main memory dependence, and low control overhead. 
Currently, systolic arrays have become the de-facto standard accelerator for highly regular DL applications, exemplified by its use in many DNN accelerators \cite{jouppi2017datacenter, XlinixDNNProcessor:online, bannon2020accelerated}.

\begin{figure}
    \center
    \includegraphics[width=0.5\textwidth]{images/Systolic.png}
    \caption{Hardware architecture of a Systolic-Array}
    \label{fig:systolic}
\end{figure}


%A systolic array \cite{kung1982systolic} defines a regular arrangement, such as a rectangular grid, of homogeneous processing elements (PEs).
%The word `systolic' implies rhythmic patterns in communication and computation, which are globally synchronous.
%This constrained dataflow restricts applications that can be mapped onto systolic arrays.
%However, the ones that can be mapped, such as matrix multiplication, have improved performance due to low control overhead and main memory dependence.
%Currently, systolic arrays have become the de-facto standard accelerator for DL applications exemplified by its use in my many DNN accelerators \cite{jouppi2017datacenter, XlinixDNNProcessor:online, bannon2020accelerated}.



% Systolic Arrays \cite{kung1982systolic} are a series of homogeneous processing elements (PE) arranged in a structural/regular order. 
% They were proposed to accelerate fairly regular computations such as matrix-multiplications. 
% The fundamental premise for systolic-arrays stem from the simple observation that memory accesses (both SRAM and DRAM) are costly, in terms of power and time, than arithmetic operations. 
% Systolic execution minimizes the costly reads and writes to the memory components by orchestrating a dataflow where each PE relies on data arriving from different directions, at regular intervals, from other neighbouring PEs, instead of the memory. 
% Currently, systolic-arrays have become the de-facto standard accelerator for DL applications. 
% This is exemplified by Tensor Processor Units (TPUs) in Google datacenters \cite{}, and the use of EdgeTPUs in mobile applications such as Google's Pixel 4 \cite{}.


\subsection{Regular Iterative and Systolic Algorithms} 
%%% ToDo: Need to make it simple without any confusion
% Systolic-algorithms are a class of algorithms that can be directly synthesized on systolic architectures. 
% Systolic architectures are limited by the dataflow, which orchestrates the computation in a structured/regular way across PEs.
% So, the mapping of algorithms onto a systolic array is limited. 
% Early research in parallel computer architecture led to developing a formal methodology to synthesize algorithms on systolic architectures/dataflow.
% The formal method constructs the computational graph for the algorithm to be mapped. 
% The computational graph contains each primitive operation as a separate node in the graph. 
% A directed edge connects the nodes if the computation at a node is dependent on another node's result.
% The computational graph is transformed into PE/Systolic architecture space to obtain the computational schedule/dataflow. 
% The computational graph could be mapped on to systolic architectures only if it has \em{constant dependency vector} \em i.e., All nodes in the graph have constant/fixed edges along each data dimension. 

%Parallelism in any algorithm can be extracted only if a language that describes that algorithm expresses the parallelism.
%Traditionally, languages are sequential and have built-in ordering that obscures the inherent parallelism present in the algorithm. 
Single-Assignment Language (SAL) \cite{gross1987mapping} provides a means of expressing parallelism in an algorithm by enforcing that no variable should be assigned a value more than once (i.e. c = c - b is not allowed). 
Regular Iterative algorithms (RIA) are a special subclass of single assignment algorithms that are specific to parallel computers with a regular array of processors, each performing the same computation and exhibiting simple inter-processor communications. Furthermore, the schedule of these algorithms onto the hardware are periodic and without control overheads. 
Systolic algorithms are a proper subclass of RIAs that contain the set of all algorithms that can be synthesized to a systolic array \cite{wan1996systolic}.
We discuss systolic algorithms with the example of matrix multiplication, as studied in the pioneering work of Kung and Leiserson \cite{kung1980systolic}.
In Fig.~\ref{fig:mm}(a) we show the standard loop implementation of a matrix-matrix multiplication. 
We transform this into the format of recurrence relations as shown in Fig.~\ref{fig:mm}(b).
These relations are said to define an RIA, since they satisfy three conditions: 
(a) Each variable is defined by a name and a set of indices (in this case 3). 
(b) Each variable is assigned a value just once (SAL \cite{gross1987mapping}). 
(c) For each recurrence relation, the difference between the indices of the variable in the LHS and each variable in the RHS is a constant.
For instance, in the equation for $C[i, j, k]$, the differences in indices (called index offsets) to the three variables $A$, $B$, and $C$ in the RHS are $[0, 0, 0], [0, 0, 0], $ and $[0, 0, -1]$, respectively.
%Systolic algorithms are RIAs that satisfy these three conditions. %RIAs that satisfy these three conditions are a super-set of algorithms which can be synthesized on systolic arrays, \textit{i.e.}, systolic algorithms.





%Parallelism in any algorithm can be extracted only if a language that describes that algorithm expresses the parallelism. 
%Traditionally, languages are sequential and have built-in ordering that obscures the inherent parallelism present in the algorithm. 
%Single-Assignment Language (SAL) \cite{} provides a means of expressing this parallelism by enforcing that every variable defined in the algorithm takes a unique value and cannot be overwritten (e.g. c = c - b is not allowed). 
%Given an SAL representation, it is possible to extract parallelism by representing the algorithm by means of a dependence graph with nodes as variables and edges as their dependencies. 
%This dependence graph specifies a partial ordering between computations of the algorithm.
%To implement the algorithm extracting parallelism on a parallel computer of processor elements, one can map the independent nodes to different processors while preserving the partial ordering. This is termed as a schedule for the computations.
%Each algorithm can have multiple schedules and determining an optimal schedule is an NP-complete problem \cite{} for the following reasons: (1) A schedule must preserve partial ordering and ensure no two computations scheduled to a processor executes at the same time, and (2) A schedule must take into account the communication constraints across processors (i.e.) time taken to transfer the dependent variables across processors. 
%
%Regular Iterative Algorithms (RIA) are a special subclass of single assignment algorithms that overcomes the difficulties of determining an optimal schedule. RIAs ensure that all computations assigned to the same processor can be described by the same simple instruction (e.g. Multiply and Accumulate). Furthermore, the schedule can be constructed to be periodic which ensures that the inter-processor communication is fixed, reducing the control overheads. Essentially, RIAs contain the set of all algorithms that can execute on a regular array of iterative processors with simple inter-processor communications. 
%
%Systolic algorithms are a proper subclass of RIAs that contain the set of all algorithms that can be synthesized to a systolic array \cite{wan1996systolic}.
%We discuss systolic algorithms with the example of matrix multiplication, as studied in the pioneering work of Kung and Leiserson \cite{kung1980systolic}.
%In Fig.~\ref{fig:mm}(a) we show the standard loop implementation of a matrix-matrix multiplication. 
%We transform this into the format of recurrence relations as shown in Fig.~\ref{fig:mm}(b).
%These relations are said to define an RIA, since they satisfy three conditions: 
%(a) Each variable is defined by a name and a set of indices (in this case 3). 
%(b) Each variable is assigned a value just once (single assignment language \cite{gross1987mapping}). 
%(c) For each recurrence relation, the difference between the indices of the variable in the LHS and each variable in the RHS is a constant.
%For instance, in the equation for $C[i, j, k]$, the differences in indices (called index offsets) to the three variables $A$, $B$, and $C$ in the RHS are $[0, 0, 0], [0, 0, 0], $ and $[0, 0, -1]$, respectively.
%RIAs that satisfy these three conditions are a super-set of algorithms which can be synthesized on systolic arrays, \textit{i.e.}, systolic algorithms.

%Regular Iterative Algorithms (RIAs) contain the set of all algorithms that can execute on a regular array of iterative processors \cite{rao1988regular}. Systolic array is a regular iterative array of Multiply and Accumulate units (MACs) and all algorithms that execute on systolic-arrays, called systolic algorithms \cite{song1994systolic}, form a proper subclass of RIA. For any algorithm, often described by a recurrence relation, to be an RIA, it has to satisfy three conditions: 
%(a) Each variable in the algorithm is assigned a value just once, (i.e.) they have to be verified to be in a single-assignment language format.  



%\subsubsection{Mapping systolic algorithms on to systolic arrays}
The computation of the said recurrence relations can be visualized geometrically as shown in Fig.~\ref{fig:mm}(c).
Each point in the 3D space corresponds to a combination of the indices $i, j, k$ starting at the origin $(0,0,0)$.
As shown, inputs $A$ and $B$ are initialized in respective planes while output $C$ is initialized with 0s. 
All values are propagated through to other points as per the recurrence relations. 
The computations for updating the values are mapped on to three dimensions.
The dimensions $i$ and $j$, along which $A$ and $B$ are propagated, are marked as systolic dimensions. 
The dimension $k$ along which $C$ is updated is marked as the `time' dimension, ending with the final computed value as shown. 
Assigning such dimensions is equivalent to \textit{mapping} the algorithm on to a 2D systolic array as shown in Fig.~\ref{fig:mm}(d).
In the mapping, matrices $A$ and $B$ are input along rows and columns (the two systolic dimensions), respectively. 
The output $C$ is computed in each processing element (PE) over time (the time dimension).
Since the output remains stationary in the PEs, this dataflow is referred to as \textit{output stationary}. 
We can similarly study input and weight stationary dataflows. 



% The computation with a variable dependency vector cannot be written in a URE/RIA and their computational graph cannot be transformed to generate a dataflow mapping/schedule.     

% The expression of a computation with a variable dependency in URE/RIA is not possible as it defies their definition.

% The computation to be mapped is represented in a recursive/iterative fashion  isto construct a computational graph with each primitive computation performed at a vertex and edges to indicate the dependence. Then, dependency vectors are computed between the points in computational graph. The algorithm with {\em constant dependency vectors} are called Systolic algorithms as they can be mapped natively to systolic architectures without requiring any transformations. A{\em constant dependency vector} indicates that there exists a constrained dataflow










%We demonstrate an example of a prominently used systolic algorithm, (i.e.) matrix multiplication. 
%\subsubsection{Matrix Multiplication}
%\begin{equation*}
%C = A \times B
%\end{equation*}
%\begin{equation*}
%0\leq i < N, 0\leq j < N, 0\leq k < N,
%\end{equation*}
%\begin{equation*}
%C(i,j,k) = C(i,j,k-1) + A(i,j,k)*B(i,j,k)
%\end{equation*}
%\begin{equation*}
%A(i,j,k) = A(i,j-1,k)
%\end{equation*}
%\begin{equation*}
%B(i,j,k) = B(i-1,j,k)
%\end{equation*}
%The dependence vectors are
%\begin{equation*}
%\theta_{A} = \begin{bmatrix}0 \\1 \\0 \\\end{bmatrix}, \theta_{B}=\begin{bmatrix}1 \\0 \\0 \\\end{bmatrix}, \theta_{C} = \begin{bmatrix}0 \\0 \\1 \\\end{bmatrix}.
%\end{equation*}



% \begin{figure}[h!] 
%     \vspace*{-5pt}
%     \centering
%     \includegraphics[width=0.4\textwidth]{images/convolutionv2.png}
%     \caption{(a) Standard spatial convolution; (b) Depth-wise separable convolution}
%     \label{fig:conv}
% \end{figure}

\subsection{Spatial and Depthwise Separable Convolutions}
% Convolution operations are common in DNNs for computer vision applications.
In \textit{spatial convolution}, an input of size $W\times H\times C$ is convolved with a filter of size $K\times K\times C$ to obtain an output of size $N\times M\times 1$, where $N=W-K+1$ and $M=H-K+1$. 
The output of $C'$ convolution filters are stacked to obtain an output of size $N\times M\times C'$.
In \textit{depthwise convolution}, an input of size $W\times H\times C$ is convolved with a filter of size $K\times K\times C$ channel-wise, \textit{i.e.}, every $W\times H$ channel is convolved with the respective $K\times K$ channel in the filter to obtain an output of size $N\times M\times C$.
This is followed by a \textit{point-wise convolution} with $C'$ filters of size $1\times 1\times C$ to obtain an output of size $N\times M\times C'$.
For both these illustrated cases, the input and output sizes are the same.
However, there is a major difference in the number of operations: Standard convolution has a total of $NMC'K^2C$ operations, while depthwise separable convolution has $NMC(K^2+C')$ operations.
This reduction in number of operations with depthwise separable convolution translates to much reduced inference time at comparable accuracy values.
%More broadly, depthwise separable convolution can be seen as a special instance of factorizing convolution \cite{szegedy2016rethinking, denton2014exploiting, lebedev2014speeding}.
%Do we need this point? 

%\subsection{Neural Architecture Search}
%NAS automates network architecture design by searching the large space of network topologies and operators. This involves a bi-level optimization -- a discrete outer-loop search for network architecture using Reinforcement Learning \cite{zoph2016neural} and Evolutionary Algorithms (EAs) \cite{real2017large}, and a continuous inner-loop optimization for weights using gradient descent. Given the expensive inner loop, NAS is compute-heavy requiring thousands of GPU-hours \cite{zoph2016neural} with alarming carbon emission levels \cite{strubell2019energy}. Several efforts have improved the efficiency of NAS by decoupling the loops \cite{cai2019once}, or using surrogate models for the inner-loop \cite{wen2020neural}. Despite the high compute costs, NAS is becoming a default choice to identify state-of-the-art DNNs for a variety of tasks.
%

% Depthwise separable convolutions are an efficient alternative for standard convolutions for mobile and embedded vision applications, popularized widely by MobileNet-V1 \cite{howard2017mobilenets}.
% %MobileNet-V1 \cite{howard2017mobilenets} proposed depthwise separable convolutions as an alternative for standard convolutions for mobile and embedded vision applications. 
% %efficient convolution for mobiles. 
% A standard convolution operation performs both filtering of inputs, and linear-combination of inputs to form new outputs in a single operation. In contrast, depthwise separable convolutions factorize standard convolutions by separating filtering and combining into two tasks - the depthwise layer and the pointwise layer respectively. 
% The depthwise layer performs filtering by applying a single $K\times K$ filter to each input channel. 
% The $1\times 1$ pointwise convolution layer takes the outputs of the depthwise layer and performs a linear-combination to form the output feature map.

% The proposed factorization reduces the required parameters, computation, and the model-size significantly. Concretely, a standard convolution with an $H\times W\times C$ feature-map and an $M\times C \times K \times K$ weight kernel, produces an output feature-map of size $H\times W\times M$\footnote{Assuming input and output feature-maps have same spatial dimensions for simplicity.}, where H and W are spatial width and height of the feature-map, K is the kernel size, C is the number of channels, and M is the number of filters. The overall computational cost for this operation is $H\times W\times C\times K\times K\times M$. 
% Whereas, upon factorizing this operation into depthwise separable convolution, the overall cost becomes $H\times W\times C \times(K\times K + M)$, a factor of $O(K^2 + M)$ reduction in the number of parameters\footnote{Actual factor is $1\setminus M + 1\setminus K^{2}$}. 
% The MobileNet architecture with depthwise separable convolutions was able to reach similar accuracies compared to MobileNet with standard convolutions (within 1\%) for an almost 10X reduction in FLOPs and 7X reduction in parameters. 
% This huge computational savings of depthwise separable convolutions enabled the rapid deployment of efficient DNNs on resource-constrained mobile/edge devices.

%A standard convolution of $H\times W\times C$ feature maps with $M\times C \times K \times K$ kernel requires a computational cost of $E\times F\times M\times K\times K\times C$. The depthwise separable convolution requires only $E \times F \times K\times K\times C$ + $E\times F\times C \times M$. The ratio of computational cost of depthwise separable convolution to standard convolution is $1\setminus M + 1\setminus K^{2}$. 
%Depthwise separable MobileNet was able to almost reach the accuracy of standard convolution MobileNet with almost 10X reduction in MACs and 7X reduction in parameters \cite{howard2017mobilenets}. 
%The huge computational savings of depth-wise separable convolutions enabled the rapid deployment of efficient DNNs on resource-constrained mobiles/edge devices.    



%Systolic Arrays \cite{kung1982systolic} are a series of homogeneous processing elements (PE) arranged in a structural/regular order. 
%Their primary objective is to reuse the data access across PEs by orchestrating a dataflow, which increases the computation throughput without any increase in memory bandwidth. 
%H.T Kung \cite{kung1982systolic} proposed ad-hoc systolic array solutions to the various computational problem such as matrix multiplication, 1D-convolution, and Fourier transforms. 
%Currently, systolic-arrays are used in Google datacenters as Tensor Processing Unit (TPU)\cite{jouppi2017datacenter,jouppi2020domain}. 
%Also, energy-constrained mobile and edge devices contain systolic arrays as EdgeTPU.




